Hypergraph Pre-training with Graph Neural Networks

Despite the prevalence of hypergraphs in a variety of high-impact applications, there are relatively few works on hypergraph representation learning, most of which primarily focus on hyperlink prediction, often restricted to the transductive learning setting. Among others, a major hurdle for effective hypergraph representation learning lies in the label scarcity of nodes and/or hyperedges. To address this issue, this paper presents an end-to-end, bi-level pre-training strategy with Graph Neural Networks for hypergraphs. The proposed framework named HyperGene bears three distinctive advantages. First, it is capable of ingesting the labeling information when available, but more importantly, it is mainly designed in the self-supervised fashion which significantly broadens its applicability. Second, at the heart of the proposed HyperGene are two carefully designed pretexts, one on the node level and the other on the hyperedge level, which enable us to encode both the local and the global context in a mutually complementary way. Third, the proposed framework can work in both transductive and inductive settings. When applying the two proposed pretexts in tandem, it can accelerate the adaptation of the knowledge from the pre-trained model to downstream applications in the transductive setting, thanks to the bi-level nature of the proposed method. The extensive experimental results demonstrate that: (1) HyperGene achieves up to 5.69% improvements in hyperedge classification, and (2) improves pre-training efficiency by up to 42.80% on average.

==> revision.tex <==
\bx{

\textbf{Notes for Experiments}:
\begin{itemize}
    \item Study the order of the node/edge pretext tasks (or what is the better way to combine them?)
    \item Tune $\alpha, \beta$ for joint training and report the best results
    \item Double-check the rationale and effectiveness of two-stage pre-training
    \item Apply other baselines from Table 3 on Amazon datasets if applicable
\end{itemize}

\textbf{Notes for Writing:}
\begin{itemize}
    \item Rephrase certain statements; pay attention to 'pretext', 'pre-training', 'self-supervised', 'contrastive'. Read the related work and try to be consistent throughout the paper
    \item Eq. (3)
    \item Is tree expansion necessary?
    \item Put the incorrectness of existing methods on constructing hypergraphs to experimental section
    \item Add more details about sampling, experimental setting, parameter tuning, and method description
\end{itemize}
}

==> timeline.tex <==
\bx{
\begin{itemize}
    \item Finish additional experiments by Dec. 28
    \item Finish the 1-st version of writing modification by Dec. 31
    \item Finish the 2-nd version by Jan. 10
    \item Keep refining the paper after the 2-nd version and add/modify experiments if necessary
\end{itemize}

}


